LIVEditor-14B: Lightning Unified Video Editing via In-Context Sparse Attention

Video editing has evolved toward In-Context Learning (ICL) paradigms, yet the resulting quadratic attention costs create a critical computational bottleneck. In this work, we propose In-context Sparse Attention (ISA), the first near-lossless empirical sparse framework tailored for ICL video editing. Our design is grounded in two key insights: first, context tokens exhibit significantly lower saliency than source tokens; second, we theoretically prove and empirically validate that Query sharpness correlates with approximation error. Motivated by these findings, ISA implements an efficient pre-selection strategy to prune redundant context, followed by a dynamic query grouping mechanism that routes high-error queries to full attention and low-error ones to a computationally efficient 0-th order Taylor sparse attention. Furthermore, we build \textbf{\texttt{LIVEditor-14B}} , a novel lightning video editing model via ISA and a proposed video-editing data pipeline that curated a 1.7M high-quality dataset. Extensive experiments demonstrate that LIVEditor-14B achieves a $\sim$60% reduction in attention-module latency while surpassing state-of-the-art methods across EditVerseBench, IVE-Bench, and VIE-Bench, delivering near-lossless acceleration without compromising visual fidelity.

==> tables/blocksize_length_ablation.tex <==
\begingroup
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
    \caption{Ablation on block size and source-sequence length on EditVerseBench (Wan2.2, default setup otherwise). Increasing block size lowers speedup while slightly improving quality; default block configuration is retained in the main experiments.}
    \label{tab:block_size_length_ablation}
    \centering
    \small
    \begin{tabular}{lcc}
        \toprule
        \textbf{Block Size} & \textbf{Tile Size} & \textbf{Quality / Speedup} \\
        \midrule
        256 & [8,8,4] & 7.69 / 1.72x \\
        64 & [4,4,4] & 7.85 / 1.47x \\
        32 (ours) & [4,4,2] & 7.89 / 1.23x \\
        8 & [2,2,2] & 7.91 / 0.29x \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[t]
    \caption{Ablation over source sequence length $L_{src}$ (Wan2.2).}
    \label{tab:source_length_ablation}
    \centering
    \small
    \begin{tabular}{ccc}
        \toprule
        $L_{src}$ & \textbf{Quality} & \textbf{Speedup} \\
        \midrule
        26,520 & 7.87 & 1.47x \\
        34,680 & 7.89 & 1.47x \\
        42,840 (ours) & 7.88 & 1.47x \\
        \bottomrule
    \end{tabular}
\end{table}
\endgroup


==> tables/channel_concat_baseline.tex <==
\begingroup
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
    \caption{Conditioning strategy comparison on Wan2.2 under comparable training settings.}
    \label{tab:channel_concat_baseline}
    \centering
    \small
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccc}
        \toprule
        \textbf{Method} & \textbf{Quality} & \textbf{Text Align} & \textbf{Temporal Consistency} & \textbf{Editing Quality} & \textbf{Pick (Frame)} & \textbf{Pick (Video)} \\
        \midrule
        Channel Concatenation Baseline & 5.69 & 18.88 & 22.43 & 18.15 & 96.57 & 97.12 \\
        ISA (Ours) & \textbf{7.89} & \textbf{20.09} & \textbf{27.19} & \textbf{24.55} & \textbf{99.32} & \textbf{99.22} \\
        \bottomrule
    \end{tabular}}
\end{table}
\endgroup


==> tables/hyvideo_comparison.tex <==
\begingroup
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
    \caption{Cross-model robustness on HunyuanVideo-1.5 using hyperparameters tuned on Wan2.2. We evaluate ISA in the training-free setting by applying it to the corresponding full-attention backbone.}
    \label{tab:hyvideo_comparison}
    \centering
    \small
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccccc}
        \toprule
        \textbf{Method} & \textbf{Quality} & \textbf{Text Align} & \textbf{Temporal Consistency} & \textbf{Editing Quality} & \textbf{Pick (Frame)} & \textbf{Pick (Video)} & \textbf{Speedup} \\
        \midrule
        Full-Attention & 6.89 & 19.42 & 26.93 & 22.15 & 98.02 & 97.92 & 1.00 \\
        ISA (Ours) & \textbf{7.04} & \textbf{19.46} & 26.89 & \textbf{22.43} & \textbf{98.16} & \textbf{98.06} & 1.39 \\
        \bottomrule
    \end{tabular}}
\end{table}
\endgroup


==> tables/teacache_compatibility.tex <==
\begingroup
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
    \caption{Compatibility with TeaCache. We report training-free results on Wan2.2 with progressively tighter temporal threshold settings $\delta$.}
    \label{tab:teacache_compatibility}
    \centering
    \small
    \begin{tabular}{lccc}
        \toprule
        \textbf{Method} & \textbf{Text Align} & \textbf{Quality} & \textbf{Speedup} \\
        \midrule
        ISA & 20.09 & 7.89 & 1.47x \\
        ISA+TeaCache ($\delta\!=\!0.10$) & 20.10 & 7.78 & 2.69x \\
        ISA+TeaCache ($\delta\!=\!0.15$) & 20.05 & 7.67 & 3.62x \\
        ISA+TeaCache ($\delta\!=\!0.20$) & 19.98 & 7.44 & 4.87x \\
        \bottomrule
    \end{tabular}
\end{table}
\endgroup

